Longitudinal double-spin asymmetry $A_1^{\rm p}$ and spin-dependent structure function $g_1^{\rm p}$ of the proton at small values of $x$ and $Q^2$

We present a precise measurement of the proton longitudinal double-spin asymmetry $A_1^{\rm p}$ and the proton spin-dependent structure function $g_1^{\rm p}$ at photon virtualities $0.006~({\rm GeV}/c)^2<Q^2 < 1~({\rm GeV}/c)^2$ in the Bjorken $x$ range of $4 \times 10^{-5} < x < 4 \times 10^{-2}$. The results are based on data collected by the COMPASS Collaboration at CERN using muon beam energies of $160~{\rm GeV}$ and $200~{\rm GeV}$. The statistical precision is more than tenfold better than that of the previous measurement in this region. In the whole range of $x$, the measured values of $A_1^{\rm p}$ and $g_1^{\rm p}$ are found to be positive. It is for the first time that spin effects are found at such low values of $x$.

==> inst_cern.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% institutes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Instfoot{bielefeld}{ Universit\"at Bielefeld, Fakult\"at f\"ur Physik, 33501 Bielefeld, Germany\Aref{f}}
\Instfoot{bochum}{ Universit\"at Bochum, Institut f\"ur Experimentalphysik, 44780 Bochum, Germany\Aref{f}}
\Instfoot{bonniskp}{ Universit\"at Bonn, Helmholtz-Institut f\"ur  Strahlen- und Kernphysik, 53115 Bonn, Germany\Aref{f}}
\Instfoot{bonnpi}{ Universit\"at Bonn, Physikalisches Institut, 53115 Bonn, Germany\Aref{f}}
\Instfoot{brno}{Institute of Scientific Instruments, AS CR, 61264 Brno, Czech Republic\Aref{g}}
\Instfoot{burdwan}{ Burdwan University, Burdwan 713104, India\Aref{i}}
\Instfoot{calcutta}{ Matrivani Institute of Experimental Research \& Education, Calcutta-700 030, India\Aref{j}}
\Instfoot{dubna}{ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia}
\Instfoot{erlangen}{ Universit\"at Erlangen--N\"urnberg, Physikalisches Institut, 91054 Erlangen, Germany\Aref{f}}
\Instfoot{freiburg}{ Universit\"at Freiburg, Physikalisches Institut, 79104 Freiburg, Germany\Aref{f}}
\Instfoot{cern}{ CERN, 1211 Geneva 23, Switzerland}
\Instfoot{heidelberg}{ Universit\"at Heidelberg, Physikalisches Institut,  69120 Heidelberg, Germany\Aref{f}}
\Instfoot{helsinki}{ Helsinki University of Technology, Low Temperature Laboratory, 02015 HUT, Finland  and University of Helsinki, Helsinki Institute of  Physics, 00014 Helsinki, Finland}
\Instfoot{licerec}{Technical University in Liberec, 46117 Liberec, Czech Republic\Aref{g}}
\Instfoot{lisbon}{ LIP, 1000-149 Lisbon, Portugal\Aref{h}}
\Instfoot{mainz}{ Universit\"at Mainz, Institut f\"ur Kernphysik, 55099 Mainz, Germany\Aref{f}}
\Instfoot{miyazaki}{University of Miyazaki, Miyazaki 889-2192, Japan\Aref{k}}
\Instfoot{moscowlpi}{Lebedev Physical Institute, 119991 Moscow, Russia}
\Instfoot{munichlmu}{Ludwig-Maximilians-Universit\"at M\"unchen, Department f\"ur Physik, 80799 Munich, Germany\Aref{f}}
\Instfoot{munichtu}{Technische Universit\"at M\"unchen, Physik Department, 85748 Garching, Germany\Aref{f}}
\Instfoot{nagoya}{Nagoya University, 464 Nagoya, Japan\Aref{k}}
\Instfoot{praguecu}{Charles University, Faculty of Mathematics and Physics, 18000 Prague, Czech Republic\Aref{g}}
\Instfoot{praguectu}{Czech Technical University in Prague, 16636 Prague, Czech Republic\Aref{g}}
%\Instfoot{aCTUa}{Czech Technical University, Faculty of Nuclear Sciences and Physical Engineering, 11519 Prague, Czech Republic\Aref{g}}
%\Instfoot{aCTUb}{Czech Technical University, Faculty of Mechanical Engineering, 16636 Prague, Czech Republic\Aref{g}}
\Instfoot{protvino}{ State Research Center of the Russian Federation, Institute for High Energy Physics, 142281 Protvino, Russia}
\Instfoot{saclay}{ CEA DAPNIA/SPhN Saclay, 91191 Gif-sur-Yvette, France}
\Instfoot{telaviv}{ Tel Aviv University, School of Physics and Astronomy, 
              %Raymond and Beverly Sackler Faculty of Exact Sciences, 
              69978 Tel Aviv, Israel\Aref{l}}
\Instfoot{triestictp}{ ICTP--INFN MLab Laboratory, 34014 Trieste, Italy}
\Instfoot{triest}{ INFN Trieste and University of Trieste, Department of Physics, 34127 Trieste, Italy}
\Instfoot{turin}{ INFN Turin and University of Turin, Physics Department, 10125 Turin, Italy}
\Instfoot{warsaw}{ So{\l}tan Institute for Nuclear Studies and Warsaw University, 00-681 Warsaw, Poland\Aref{m} }
\Instfoot{warsawtu}{ Warsaw University of Technology, Institute of Radioelectronics, 00-665 Warsaw, Poland\Aref{n} }
\Anotfoot{a}{Also at IST, Universidade T\'ecnica de Lisboa, Lisbon, Portugal}
\Anotfoot{b}{Also at University of East Piedmont, 15100 Alessandria, Italy}
\Anotfoot{c}{On leave of absence from JINR Dubna}               
\Anotfoot{d}{Also at Chubu University, Kasugai, Aichi, 487-8501 Japan}
\Anotfoot{e}{Also at Yamagata University, Yamagata, 992-8510 Japan}
\Anotfoot{f}{Supported by the German Bundesministerium f\"ur Bildung und Forschung}
\Anotfoot{g}{Suppported by Czech Republic MEYS grants ME492 and LA242}
\Anotfoot{h}{Supported by the Portuguese FCT - Funda\c{c}\~ao para
               a Ci\^encia e Tecnologia grants POCTI/FNU/49501/2002 and POCTI/FNU/50192/2003}
\Anotfoot{i}{Supported by DST-FIST II grants, Govt. of India}
\Anotfoot{j}{Supported by  the Shailabala Biswas Education Trust}
\Anotfoot{k}{Supported by the Ministry of Education, Culture, Sports,
               Science and Technology, Japan; Daikou Foundation and Yamada Foundation}
\Anotfoot{l}{Supported by the Israel Science Foundation, founded by the Israel Academy of Sciences and Humanities}
\Anotfoot{m}{Supported by KBN grant nr 621/E-78/SPUB-M/CERN/P-03/DZ 298 2000,
               nr 621/E-78/SPB/CERN/P-03/DWM 576/2003-2006, and by MNII reasearch funds for 2005--2007}
\Anotfoot{n}{Supported by  KBN grant nr 134/E-365/SPUB-M/CERN/P-03/DZ299/2000}


